Attention-Based Neural Networks for Sentiment Attitude Extraction using Distant Supervision

In the sentiment attitude extraction task, the aim is to identify <<attitudes>> -- sentiment relations between entities mentioned in text. In this paper, we provide a study on attention-based context encoders in the sentiment attitude extraction task. For this task, we adapt attentive context encoders of two types: (1) feature-based; (2) self-based. In our study, we utilize the corpus of Russian analytical texts RuSentRel and automatically constructed news collection RuAttitudes for enriching the training set. We consider the problem of attitude extraction as two-class (positive, negative) and three-class (positive, negative, neutral) classification tasks for whole documents. Our experiments with the RuSentRel corpus show that the three-class classification models, which employ the RuAttitudes corpus for training, result in 10% increase and extra 3% by F1, when model architectures include the attention mechanism. We also provide the analysis of attention weight distributions in dependence on the term type.

==> parts/acknowledgments.tex <==
\section*{Acknowledgments}
The reported study was funded by RFBR according to the research project \textnumero~20-07-01059. 

% The reported study was funded by RFBR according to the research project \textnumero~19-37-50001. 
% The development of Russian sentiment frames is supported by the RFBR research project \textnumero~16-29-09606.

==> parts/review_parts/rusentrel.tex <==
% RuSentRel
A corpus of analytical articles, obtained from authoritative foreign sources and translated 
into Russian, has been compiled in~\cite{loukachevitch2018extracting}.
The collected articles contain both the author's opinion on the subject matter
of the article and a large number of attitudes mentioned between the participants of the 
described situations.
In total, 73 large analytical texts were labeled with about 2000 relations.
The authors experimented with automatic attitude extraction using the developed corpus.
In comparison with~\cite{choi2016document}, where documents are much smaller and written in English,
the authors obtained similar F-measure and concluded that the task still remains complicated.

